Decoupling Shrinkage and Selection for the Bayesian Quantile Regression

This paper extends the idea of decoupling shrinkage and sparsity for continuous priors to Bayesian Quantile Regression (BQR). The procedure follows two steps: In the first step, we shrink the quantile regression posterior through state of the art continuous priors and in the second step, we sparsify the posterior through an efficient variant of the adaptive lasso, the signal adaptive variable selection (SAVS) algorithm. We propose a new variant of the SAVS which automates the choice of penalisation through quantile specific loss-functions that are valid in high dimensions. We show in large scale simulations that our selection procedure decreases bias irrespective of the true underlying degree of sparsity in the data, compared to the un-sparsified regression posterior. We apply our two-step approach to a high dimensional growth-at-risk (GaR) exercise. The prediction accuracy of the un-sparsified posterior is retained while yielding interpretable quantile specific variable selection results. Our procedure can be used to communicate to policymakers which variables drive downside risk to the macro economy.

==> Chapters/Global_Local_Priors.tex <==
In order to identify the posterior of a large dimensional coefficient vector in small samples, informative priors are needed. Ideally, these priors are able to separate noise variables from signals such that the noise is shrunk towards zero and signals attain their unrestricted parameter values. Global-local priors are continuous shrinkage priors which share the trait that their marginal prior distribution on the regression coefficients provide large mass on zero (typically far more than the normal distribution) and fat tails which allow for signals with large coefficients to escape shrinkage \citep{polson2010shrink}. The general class of global-local priors takes the following form:
\begin{equation} \label{eq:gl}
\begin{split}
     \beta_j | \lambda_j^2, \nu^2, \sigma^2 & \sim N(0,\lambda_j^2\nu^2), j \in (1,\cdots, K) \\
    \lambda_j & \sim \pi(\lambda_j)d\lambda_j, j \in (1,\cdots, K) \\
    \nu & \sim \pi(\nu)d\nu.
    \end{split}
\end{equation}
The global scale-prior $\nu^2$, controls the overall shrinkage applied to the coefficients and a local scale $\lambda^2_j$ allows for the local possibility of regressors to escape shrinkage when they have large effects on the response. In order to achieve this flexibility in shrinkage and good separation between noise and signal variables, GL priors employ very fat-tailed distributions for both the global and local prior. The horseshoe prior of \citet{carvalho2010horseshoe}, employs two half Cauchy distributions for $\lambda_j$ and $\nu$:
\begin{equation}  \label{prior5}
 \begin{split}
     \lambda_j^2 & \sim C_+(0,1) \\
     \nu^2 & \sim C_+(0,1).
 \end{split}
 \end{equation}
Recent work of [citation] have found that the horseshoe prior achieves near minimax rates in posterior consistency in high dimensional regression problems and has the additional advantage of not needing any further hyperparameters.

[The Lasso prior]

[The SSVS prior]


==> Chapters/HS_augmented_BQR.tex <==
In order to generalize the horseshoe prior to the ALL in (\ref{worklik}), it needs to be formulated under the assumption of independence between the $\beta$ and $\sigma$ prior so that the posterior takes a conditionally normal form \citep{kozumi2011gibbs}. While prior independence between regression coefficients and error variance might seem like a strong assumption, \cite{moran2018variance} have shown that in high-dimensional settings, the independence assumption aids inference of the error variance. This is due to the fact that conjugate priors act mathematically as additional observations which artificially bias the error variances downwards when K$>>$T. 

The general independent global-local prior takes the following hierarchical form: 
 \begin{equation} \label{prior1}
 \begin{split}
    \sigma^2 & \sim \pi(\sigma^2)d\sigma^2 \\
    \beta_j | \lambda_j^2, \nu^2 & \sim N(0,\lambda_j^2\nu^2), j \in (1,\cdots, K) \\
    \lambda_j^2 & \sim \pi(\lambda_j^2)d\lambda_j^2, j \in (1,\cdots, K) \\
    \nu^2 & \sim \pi(\nu^2)d\nu^2
    \end{split}
    \end{equation}

As recommended by \cite{gelman2006prior}, we select a weakly informative inverse Gamma distribution as the prior for the error variance $\sigma^2$ instead of non-informative priors and two independently distributed half Cauchy distributions on the positive support for the scale parameters of the $\beta$ prior:
 \begin{equation} \label{prior2}
  \sigma^2 \sim IG(\underline{a},\underline{b})   
 \end{equation}
 \begin{equation}  \label{prior3}
     \lambda_j^2 \sim C_+(0,1)
 \end{equation}
 \begin{equation}  \label{prior4}
    \nu^2 \sim C_+(0,1)     
 \end{equation}
Under the above priors, the posteriors take the following form:
 \begin{equation} \label{postbeta}
     \beta|\sigma, X, Y, Z \sim N(\overline{\beta}. \overline{V}),
 \end{equation}
where $\overline{V}= (X'UX+\underline{V})^{-1}, U=diag(\frac{1}{\tau^2z_i\sigma})$ and $\underline{V}=\nu^2diag(\lambda^2_1,\cdots,\lambda^2_K)$, and $\overline{\beta}$ is defined as $\overline{\beta}=(X'UX+\overline{V}^{-1})^{-1}(X'Uy+\overline{V}^{-1}\underline{\beta})$ with $\underline{\beta}=\boldsymbol{0}_K$. The conditional posterior of the scale parameter is given by
\begin{equation}
    \sigma^2|\beta, X, Y, Z \sim IG(\overline{a},\overline{b})
\end{equation}
and $\overline{a}=\underline{a}+\frac{3T}{2}$, $\overline{b}=\underline{b}+\sum_{t=1}^T\frac{(y_t-x_t'\beta-\theta z_t))^2}{2z_t+\tau^2}+\sum_{t=1}^Tz_t$. 

Due to the assumption of independence on the scales $(\lambda,\nu)$, it is straightforward to show that their posteriors follow independent Cauchy distributions. Since the Cauchy has no defined moments which would enable sampling, the literature has proposed Gibbs samplers which rely either on slice sampling \citep{polson2014bayesian} or mixture representations \citep{makalic2015simple}. Unfortunately, both rely on conjugate formulations. We use the fact that the posterior distribution of $\lambda_j$ conditional on $\nu$ remains independent of all other parameters by assumption, to formulate a block slice sampling algorithm for for $\lambda=(\lambda_1,\cdots,\lambda_K)'$ akin to \cite{polson2014bayesian} which is given in \ref{Slicesampling}. Finally, since the latent $z_t$ are sampled independently, the conditional posterior follows the reciprocal of the inverse Gaussian:
\begin{equation}
    z_t|\beta,\sigma,X,Y\sim I-G(\overline{c_t},\overline{d_t})
\end{equation}
Where I-G stands for the inverse Gaussian distribution with location and rate parameters respectively, $\overline{c_t}=\frac{\sqrt{\theta^2+2\tau^2}}{|y_t-x_t'\beta|}$ and $\overline{d_t}=\frac{\theta^2+2\tau^2}{\sigma\tau^2}$. \\

\subsection{Gibbs Sampler}

With these conditional posteriors at hand, we utilize a standard Gibbs sampler. The dynamics of the Markov chain  $\{(\beta_m,\sigma_m,\lambda^2_m,\nu^2_m,z_{m})\}_{m=0}^{\infty}$ are implicitly defined through the following steps
    \begin{enumerate}
        \item Draw $Z \sim \pi(.|\beta,\sigma,\lambda^2,\nu^2,\theta,\tau,X,Y)$ from I-G($\overline{c_t}$,$\overline{d_t}$) for all t and call the T x 1 vector $z_{n+1}$
        \item Draw $\sigma_{n+1} \sim \pi(.|\beta,\lambda^2, \nu^2,\theta,\tau,X,Y,z_{n+1}) $ from $IG (\overline{a},\overline{b})$
        \item Draw $\beta_{n+1} \sim \pi(.|\sigma_{n+1},\lambda^2,\nu^2,\theta,\tau,X,Y,z_{n+1})$ from $N(\overline{\beta},\overline{V})$
        \item Simulate $\lambda^2_{n+1}$ and $\nu^2_{n+1}$ through slice sampling as in \ref{Slicesampling}
        \item Iterate (1-4) until convergence is achieved
    \end{enumerate}

\cite{khare2012geometric} show that the Markov chain of this sampler is geometrically ergodic and also valid in K$>>$T settings which gives theoretical justification to apply this sampler to high dimensional settings. However, a computational bottleneck is present in very high dimensions in evaluating the $K\times K$ dimensional inverse for the conditional posterior of $\beta$. Cholesky decomposition based methods will generally be of order $O(K^3)$. Taking into consideration that in quantile settings, one is usually interested in obtaining more than one expected quantile, this can result in prohibitively long computation times. We therefore provide a more efficient sampling algorithm for $\beta$ which leverages data augmentation similar to the algorithm developed by \cite{bhattacharya2016fast} which is of order $O(T^2K)$ and especially beneficial in high dimensional settings.

As derived above, using the scale mixture representation in (\ref{prior1}), the conditional posterior of $\beta$ given all other parameters can be written as:
\begin{equation} \label{proof1}
    \beta | \sigma, X, Y,Z \sim N(A^{-1}X'Uy, A^{-1}), \quad A = (X'UX + \Lambda_{*}^{-1}), \quad \Lambda_{*}^{-1} = \nu^2 diag(\lambda_1^2,\cdots,\lambda_K^2)  
\end{equation}

Suppose, we want to sample from $N_K(\mu, \Sigma)$, where
\begin{equation} \label{proof2}
    \Sigma = (\Phi'\Phi + D)^{-1}, \quad \mu=\Sigma\Phi'\alpha.    
\end{equation}

Assume $D \in \mathbb{R}^{K \times K}$ is a positive definitive matrix, $\boldsymbol{\phi} \in \mathbb{R}^{T \times K}$, and $\alpha \in \mathbb{R}^{T \times 1}$. Then (\ref{proof1}) is a special case of of (\ref{proof2}) when setting $\Phi=\sqrt{U}X$, $D=\Lambda_{*}$ and $\alpha=\sqrt{U}y$. An exact algorithm to sample from (\ref{proof1}) is thus given by:

\newmdtheoremenv{theo}{Algorithm}
\begin{theo}
Fast HS-BQR sampler
\begin{enumerate}
    \item Sample independently $u \sim N(0,D)$ and $\delta \sim N(0,I_T)$
    \item Set $\xi=\Phi u + \delta$
    \item Solve $(\Phi D \Phi' + I_T)w=(\alpha - \xi)$
    \item Set $\theta = u + D\Phi'w$
\end{enumerate}
\end{theo}

\begin{flushleft}

\textbf{Proposition} \textit{Suppose $\theta$ is obtained through algorithm 1. Then $\theta\sim N(\mu, \Sigma)$}. \\
\end{flushleft}
\textit{Proof.} Using the Sherman-Morrison-Woodbury identity, $\mu=D\Phi'(\Phi D \Phi' + I_T)^{-1}\alpha$. Plugging in 2. into 3., we obtain $\theta = u + D\Phi'(\Phi D \Phi'+I_T)^{-1}(\alpha-\xi)$. Since by definition $\xi \sim N(0,\Phi D \Phi + I_K)$, $\theta$ follows a normal distribution with mean $D \Phi'(\Phi D \Phi'+ I_K)\alpha=\mu$. As $cov(u,\xi)=D \Phi'$, it follows that $cov(\theta)=D-D \Phi'(\Phi D \Phi' + I_K)^{-1}\Phi D$ which by the Sherman-Morrison-Woodbury identity is equal to $\Sigma$. More details are provided in (\ref{Algorithm}). The provided algorithm is not specific to the horseshoe prior and follows through for any prior of the form in (\ref{prior1}). The computational advantage provided in algorithm 1 compared to Cholesky based decompositions is that we can cheaply sample from $(u,\xi)'$ which via data augmentation yields samples from the desired distributions. 
